Slick: Secure Middleboxes using Shielded Execution

Cloud computing offers the economies of scale for computational resources with the ease of management, elasticity, and fault tolerance. To take advantage of these benefits, many enterprises are contemplating to outsource the middlebox processing services in the cloud. However, middleboxes that process confidential and private data cannot be securely deployed in the untrusted environment of the cloud. To securely outsource middleboxes to the cloud, the state-of-the-art systems advocate network processing over the encrypted traffic. Unfortunately, these systems support only restrictive middlebox functionalities, and incur prohibitively high overheads due to the complex computations involved over the encrypted traffic. This motivated the design of Slick --- a secure middlebox framework for deploying high-performance Network Functions (NFs) on untrusted commodity servers. Slick exposes a generic interface based on Click to design and implement a wide-range of NFs using its out-of-the box elements and C++ extensions. Slick leverages SCONE (a shielded execution framework based on Intel SGX) and DPDK to securely process confidential data at line rate. More specifically, Slick provides hardware-assisted memory protection, and configuration and attestation service for seamless and verifiable deployment of middleboxes. We have also added several new features for commonly required functionalities: new specialized Click elements for secure packet processing, secure shared memory packet transfer for NFs chaining, secure state persistence, an efficient on-NIC timer for SGX enclaves, and memory safety against DPDK-specific Iago attacks. Furthermore, we have implemented several SGX-specific optimizations in Slick. Our evaluation shows that Slick achieves near-native throughput and latency.

==> fig-system-thread-design.tex <==
\begin{figure}[t]
\centering

\includegraphics[width=\columnwidth]{figures/}

\caption{NFVs chaining in \slick}

\label{fig:nfv-chains}
\end{figure}

